Safe and Compliant Control of Redundant Robots Using Superimposition of Passive Task-Space Controllers

Safe and compliant control of dynamic systems in interaction with the environment, e.g., in shared workspaces, continues to represent a major challenge. Mismatches in the dynamic model of the robots, numerical singularities, and the intrinsic environmental unpredictability are all contributing factors. Online optimization of impedance controllers has recently shown great promise in addressing this challenge, however, their performance is not sufficiently robust to be deployed in challenging environments. This work proposes a compliant control method for redundant manipulators based on a superimposition of multiple passive task-space controllers in a hierarchy. Our control framework of passive controllers is inherently stable, numerically well-conditioned (as no matrix inversions are required), and computationally inexpensive (as no optimization is used). We leverage and introduce a novel stiffness profile for a recently proposed passive controller with smooth transitions between the divergence and convergence phases making it particularly suitable when multiple passive controllers are combined through superimposition. Our experimental results demonstrate that the proposed method achieves sub-centimeter tracking performance during demanding dynamic tasks with fast-changing references, while remaining safe to interact with and robust to singularities. he proposed framework achieves such results without knowledge of the robot dynamics and thanks to its passivity is intrinsically stable. The data further show that the robot can fully take advantage of the redundancy to maintain the primary task accuracy while compensating for unknown environmental interactions, which is not possible from current frameworks that require accurate contact information.

==> ToDoList.tex <==
\section*{To do list}
\begin{itemize}
    \item Finalise Simulations Method
    \item Add a figure with task-space controllers representation
    \item Revise Introduction to be aligned with final message
    \item Run Simulations and Write Results down results
    \item Write Discussion, Conclusion and Abstract
    \item (Gazebo) Check if we should add the viscous dissipation as in \cite{babarahmati2019} to account for model errors
\end{itemize}

\section*{Potential contributions}
\begin{itemize}
    \item \cite{babarahmati2019} uses a fixed null-space resolution term in Alg. 1. Here, we use a Stack of FICs to get around the null-space resolution.
    \item "Claim increase robustness to unpredicted/unknown obstacles. Obviously, the target has to be within the reach of the terminal part of the manipulator"
    \item tbc: Dealing with orientations - we may want to look into this closer
    \item Model-free impedance controller - to the best of our knowledge the first implementation/demonstration of this [comparison to previous: Previous used a model-based gravity compensation; our work does not. It can also be used to play arbitrary trajectories]
\end{itemize}

==> figures/fig-hw-ee-velocities.tex <==
\begin{figure*}[t]
    \begin{subfigure}[t]{0.245\linewidth}
        \includegraphics[width=\linewidth,trim={0.1in 0.1in 0.12in 0.1in},clip]{8_NoI/1_ee_ref_velocity.pdf}
        \caption{Figure 8, no interaction}
    \end{subfigure}
    \begin{subfigure}[t]{0.245\linewidth}
        \includegraphics[width=\linewidth,trim={0.1in 0.1in 0.12in 0.1in},clip]{8_WInt/1_ee_ref_velocity.pdf}
        \caption{Figure 8, with interaction}
    \end{subfigure}
    \begin{subfigure}[t]{0.245\linewidth}
        \includegraphics[width=\linewidth,trim={0.1in 0.1in 0.12in 0.1in},clip]{StrL_NoI/1_ee_ref_velocity.pdf}
        \caption{Straight-line, no interaction}
    \end{subfigure}
    \begin{subfigure}[t]{0.245\linewidth}
        \includegraphics[width=\linewidth,trim={0.1in 0.1in 0.12in 0.1in},clip]{StrL_WInt/1_ee_ref_velocity.pdf}
        \caption{Straight-line, with interaction}
    \end{subfigure}
    \caption{\emph{Hardware experiments:} Changes to the reference for the end-effector passed to the Stack of Passive Controllers framework for each of the experiments.}
\end{figure*}

